Scaling GR(1) Synthesis via a Compositional Framework for LTL Discrete Event Control

We present a compositional approach to controller synthesis of discrete event system controllers with linear temporal logic (LTL) goals. We exploit the modular structure of the plant to be controlled, given as a set of labelled transition systems (LTS), to mitigate state explosion that monolithic approaches to synthesis are prone to. Maximally permissive safe controllers are iteratively built for subsets of the plant LTSs by solving weaker control problems. Observational synthesis equivalence is used to reduce the size of the controlled subset of the plant by abstracting away local events. The result of synthesis is also compositional, a set of controllers that when run in parallel ensure the LTL goal. We implement synthesis in the MTSA tool for an expressive subset of LTL, GR(1), and show it computes solutions to that can be up to 1000 times larger than those that the monolithic approach can solve.

==> sections/renaming.tex <==

%%%%% RENAMING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Renaming preserves controllability 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Renaming}
\label{subsection:renaming}
The theorem above requires the result of quotienting one of the LTS in $\mathcal{M}$ (i.e., $M_{1}^{c} \slash \! \sim_\Upsilon$) to be deterministic. This is not always the case but can be achieved by first renaming any events that may introduce non-determinism.

We use \textit{renaming} to disambiguate nondeterminism as in \cite{wong1989computation}. 

\begin{definition}[Renaming]
Let $\Sigma_1$, $\Sigma_2$ two sets of events and $\Sigma_c$ a set of controllable events. We define $\rho: \ \Sigma_2 \xrightarrow[]{} \Sigma_1$ as a \textit{renaming} which \textit{preserves controllability of labels} (i.e., if $a \in \Sigma_2$, then $\rho(a) \in \Sigma_c$  iff $a \in \Sigma_c$).
\end{definition} 

Renaming to avoid nondeterminism will introduce new events. Thus controllers with a different alphabet from that of the original plant will be synthesised. This entails that, when the plant exhibits an event $e \in \Sigma$, we have to determine which of the new events $e' \in \rho(\Sigma)$ should be triggered in the controller. This is achieved using a \textit{distinguisher}\cite{mohajerani_framework_2014}.

\begin{definition}[$\rho$-\textit{distinguisher} \cite{mohajerani_framework_2014}]
Let $\rho: \ \Sigma_2 \xrightarrow[]{} \Sigma_1$ be a renaming. An LTS $D$ with alphabet $\Sigma_2$ is a $\rho$-\textit{distinguisher} if, for all traces $s, t \in \mathcal{L}(D)$,  $\rho(s) = \rho(t)$, implies $s = t$.
\end{definition}

Renaming with $\rho$-distinguishers  guarantees that only one of the renamed events is enabled in each state. \vb{No entiendo la frase anterior. No me compila.  El renaming está hecho con una función no con un automata. para empezar, además no entiendo el significado. }


\begin{definition}[Reverse renaming]\cite{mohajerani_framework_2014}
\label{def:reverse_renaming}
Let $M = (S_{M}, \Sigma_1, \xrightarrow[]{}_M, s_{M_0})$ be an LTS, and let $\rho: \Sigma_2 \xrightarrow{} \Sigma_1$ be a renaming. Then $\rho^{-1}(M) = (S_M, \Sigma_2, \xrightarrow[]{}_{\rho^{-1}}, s_{M_0})$ where $x \xrightarrow[]{\sigma}_{\rho^{-1}} y$ iff $x \xrightarrow[]{\rho(\sigma)} y$.

\end{definition}


The following theorem states that renaming can be applied to a synthesis tuple without changing its solutions.  The proof follows from \cite{mohajerani_framework_2014}.

\begin{theorem}[Renaming preserves controllers]
    Let $\varphi$ a GR(1) formula, $\Sigma_c \subseteq \Sigma$ a set of controllable events, $\mu$ a set of uncontrollable events, $\mathcal{M} = \{ M_1, .., M_n \}$, let $D$ be a $\rho$-distinguisher such that $\rho(D)=M_1$ and $\mathcal{M'} = \{ D, \rho^{-1}(M_2), .., \rho^{-1}(M_n) \}$. Then $(\mathcal{M}, \mathcal{C}, \rho_{1}, \mu) \cong_{\Sigma_c, \varphi} (\mathcal{M'}, \rho^{-1}(\mathcal{C}) \cup \{ D \}, \rho_{1} \circ \rho, \mu)$
\end{theorem}

